Scheduling Refresh Queries for Keeping Results from a SPARQL Endpoint Up-to-Date (Extended Version)

Many datasets change over time. As a consequence, long-running applications that cache and repeatedly use query results obtained from a SPARQL endpoint may resubmit the queries regularly to ensure up-to-dateness of the results. While this approach may be feasible if the number of such regular refresh queries is manageable, with an increasing number of applications adopting this approach, the SPARQL endpoint may become overloaded with such refresh queries. A more scalable approach would be to use a middle-ware component at which the applications register their queries and get notified with updated query results once the results have changed. Then, this middle-ware can schedule the repeated execution of the refresh queries without overloading the endpoint. In this paper, we study the problem of scheduling refresh queries for a large number of registered queries by assuming an overload-avoiding upper bound on the length of a regular time slot available for testing refresh queries. We investigate a variety of scheduling strategies and compare them experimentally in terms of time slots needed before they recognize changes and number of changes that they miss.

==> main-gnuplottex-fig1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7488.00,3456.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%
      \put(550,927){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(550,1304){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(550,1682){\makebox(0,0)[r]{\strut{}2}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(550,2059){\makebox(0,0)[r]{\strut{}3}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(550,2436){\makebox(0,0)[r]{\strut{}4}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(550,2814){\makebox(0,0)[r]{\strut{}5}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(550,3191){\makebox(0,0)[r]{\strut{}6}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(729,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/01}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1133,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/08}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1537,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/15}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1941,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/22}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2344,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/29}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2748,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/05}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3152,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/12}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3556,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/19}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3960,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/26}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4364,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/03}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4768,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/10}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5171,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/17}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5575,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/24}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5979,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/31}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6211,1153){\makebox(0,0)[l]{\strut{}396}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6211,1606){\makebox(0,0)[l]{\strut{}398}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6211,2059){\makebox(0,0)[l]{\strut{}400}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6211,2512){\makebox(0,0)[l]{\strut{}402}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6211,2965){\makebox(0,0)[l]{\strut{}404}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2059){\rotatebox{-270}{\makebox(0,0){\strut{}triples +/- ($10^5$)}}}%
      \put(6980,2059){\rotatebox{-270}{\makebox(0,0){\strut{}triples total ($10^6$)}}}%
      \csname LTb\endcsname%
      \put(5045,3018){\makebox(0,0)[r]{\strut{}deleted}}%
      \csname LTb\endcsname%
      \put(5045,2798){\makebox(0,0)[r]{\strut{}inserted}}%
      \csname LTb\endcsname%
      \put(5045,2578){\makebox(0,0)[r]{\strut{}total}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{main-gnuplottex-fig1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> main-gnuplottex-fig2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7488.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,927){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,1261){\makebox(0,0)[r]{\strut{}50}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,1596){\makebox(0,0)[r]{\strut{}100}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,1930){\makebox(0,0)[r]{\strut{}150}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,2265){\makebox(0,0)[r]{\strut{}200}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,2599){\makebox(0,0)[r]{\strut{}250}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,2934){\makebox(0,0)[r]{\strut{}300}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(682,3268){\makebox(0,0)[r]{\strut{}350}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(861,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/01}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1257,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/08}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1653,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/15}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2048,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/22}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2444,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/29}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2840,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/05}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3236,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/12}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3631,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/19}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4027,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/26}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4423,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/03}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4819,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/10}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5215,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/17}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5610,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/24}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6006,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/31}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2131){\rotatebox{-270}{\makebox(0,0){\strut{}changed query results}}}%
      \csname LTb\endcsname%
      \put(5071,2131){\makebox(0,0)[r]{\strut{}total distinct changed queries}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,927){\makebox(0,0)[l]{\strut{}0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,1271){\makebox(0,0)[l]{\strut{}5}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,1615){\makebox(0,0)[l]{\strut{}10}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,1959){\makebox(0,0)[l]{\strut{}15}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,2303){\makebox(0,0)[l]{\strut{}20}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,2647){\makebox(0,0)[l]{\strut{}25}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,2991){\makebox(0,0)[l]{\strut{}30}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6626,3335){\makebox(0,0)[l]{\strut{}35}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{main-gnuplottex-fig2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> main-gnuplottex-fig3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7488.00,3600.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%
      \put(814,927){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(814,1730){\makebox(0,0)[r]{\strut{}10}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(814,2532){\makebox(0,0)[r]{\strut{}100}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(814,3335){\makebox(0,0)[r]{\strut{}1000}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(993,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/01}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1380,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/08}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1767,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/15}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2153,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/22}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2540,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/29}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2927,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/05}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3314,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/12}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3701,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/19}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4087,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/26}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4474,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/03}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4861,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/10}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5248,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/17}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5635,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/24}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6021,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/31}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2131){\rotatebox{-270}{\makebox(0,0){\strut{}queries runtime (sec) in log-10}}}%
      \csname LTb\endcsname%
      \put(5070,2906){\makebox(0,0)[r]{\strut{}total runtime}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6631,927){\makebox(0,0)[l]{\strut{}0}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6631,1328){\makebox(0,0)[l]{\strut{}10}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6631,1729){\makebox(0,0)[l]{\strut{}20}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6631,2131){\makebox(0,0)[l]{\strut{}30}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6631,2532){\makebox(0,0)[l]{\strut{}40}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6631,2933){\makebox(0,0)[l]{\strut{}50}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6631,3335){\makebox(0,0)[l]{\strut{}60}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{main-gnuplottex-fig3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> main-gnuplottex-fig4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,1064){\makebox(0,0)[r]{\strut{}114325}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,1202){\makebox(0,0)[r]{\strut{}118203}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,1339){\makebox(0,0)[r]{\strut{}118603}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,1477){\makebox(0,0)[r]{\strut{}123957}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,1614){\makebox(0,0)[r]{\strut{}124319}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,1752){\makebox(0,0)[r]{\strut{}129276}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,1889){\makebox(0,0)[r]{\strut{}132249}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2026){\makebox(0,0)[r]{\strut{}133188}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2164){\makebox(0,0)[r]{\strut{}134116}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2301){\makebox(0,0)[r]{\strut{}140461}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2439){\makebox(0,0)[r]{\strut{}145265}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2576){\makebox(0,0)[r]{\strut{}147471}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2714){\makebox(0,0)[r]{\strut{}148158}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2851){\makebox(0,0)[r]{\strut{}149553}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,2988){\makebox(0,0)[r]{\strut{}152280}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,3126){\makebox(0,0)[r]{\strut{}155182}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,3263){\makebox(0,0)[r]{\strut{}156903}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,3401){\makebox(0,0)[r]{\strut{}330188}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,3538){\makebox(0,0)[r]{\strut{}330403}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,3676){\makebox(0,0)[r]{\strut{}330809}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,3813){\makebox(0,0)[r]{\strut{}339134}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,3950){\makebox(0,0)[r]{\strut{}340269}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,4088){\makebox(0,0)[r]{\strut{}341965}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,4225){\makebox(0,0)[r]{\strut{}342431}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,4363){\makebox(0,0)[r]{\strut{}342435}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,4500){\makebox(0,0)[r]{\strut{}422350}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,4638){\makebox(0,0)[r]{\strut{}422789}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{}425732}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1257,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/01}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(1679,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/08}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2102,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/15}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2524,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/22}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(2946,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}08/29}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3369,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/05}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(3791,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/12}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4214,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/19}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(4636,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}09/26}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5058,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/03}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5481,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/10}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(5903,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/17}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6325,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/24}}}%
      \colorrgb{0.50,0.50,0.50}%
      \put(6748,748){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}10/31}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2851){\rotatebox{-270}{\makebox(0,0){\strut{}LSQ query id}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{main-gnuplottex-fig4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> sections/notes.tex <==
\section*{Notes}

\iffalse
SELECT qe1.`query_id`, qe1.`result_size`, qe2.`result_size`
FROM `query_execution` AS qe1, `query_execution` AS qe2
WHERE qe1.`query_id` = qe2.`query_id` AND qe1.`revision_id` = qe2.`revision_id` - 1
AND qe1.`result_size` != qe2.`result_size`;

SELECT COUNT(`query_id`) AS queries, `revs`
FROM (SELECT `query_id`, COUNT(`revision_id`) AS revs
      FROM `query_execution`
      GROUP BY `query_id`) AS r
GROUP BY `revs`;

SELECT `revision_id`, SUM(`run_time_ms`) AS ms, SUM(`run_time_ms`)/1000/60 AS min
FROM `query_execution`
GROUP BY `revision_id`
ORDER BY `revision_id`;

SELECT `query_id`, `revision_id`, `result_change`, `result_size`
FROM `query_execution`
WHERE `query_id` IN (SELECT DISTINCT `query_id` FROM `query_execution` WHERE `result_change` = true)
ORDER BY `query_id`, `revision_id`;

SELECT DISTINCT `query_id`, `url`, `text`, `type`, `ordered`, `result_limit`, `result_offset` FROM `query_execution`, `query`  WHERE `query_execution`.`query_id` = `query`.`id` AND `result_change` = true;

SELECT COUNT(DISTINCT `query_id`), `type` FROM `query_execution`, `query`  WHERE `query_execution`.`query_id` = `query`.`id` AND `result_change` = true GROUP BY `type`;

SELECT config, strategy, COUNT(DISTINCT revision_id) AS revs, 
  COUNT(query_id) AS query_execs, COUNT(DISTINCT query_id) AS queries, 
  SUM(delay) AS delay_total, AVG(delay), MAX(delay), -- SUM(CASE WHEN delay > 0 THEN 1 ELSE 0 END) AS `delayed`, SUM(delay) / SUM(change_detection) AS `delay_avg`,
  SUM(missed_n) AS missed_total, AVG(missed_n), MAX(missed_n), -- SUM(CASE WHEN missed_n > 0 THEN 1 ELSE 0 END) AS missed, SUM(missed_n) / SUM(change_detection) AS missed_avg, 
  SUM(change_detection) AS changed -- , MAX(max_runtime)
FROM `evaluation`
WHERE config="maxRuntime=50000,maxRev=1000"
-- "maxRuntime=10000,maxRev=588"
GROUP BY config, strategy -- , revision_id
ORDER BY config, strategy

\fi
